Real-time Collaborative Multi-Level Modeling by Conflict-Free Replicated Data Types

The need for real-time collaborative solutions in model-driven engineering has been increasing over the past years. Conflict-free replicated data types (CRDT) provide scalable and robust replication mechanisms that align well with the requirements of real-time collaborative environments. In this paper, we propose a real-time collaborative multi-level modeling framework to support advanced modeling scenarios, built on a collection of custom CRDT, specifically tailored for the needs of modeling environments. We demonstrate the benefits of the framework through an illustrative modeling case and compare it with other state-of-the-art modeling frameworks.

==> bio/bio.tex <==
\textbf{Istvan David} is a Postdoctoral Research Fellow at the Department of Computer Science and Operations Research at the University of Montreal, Canada. He received his PhD in Computer Science from the University of Antwerp, Belgium. His research focuses on collaborative modeling, multi-paradigm modeling and model transformations. Istvan is an IVADO Postdoctoral Research Scholarship laureate on the topic of inference of simulation models in digital twins by reinforcement learning. Contact him at http://istvandavid.com.

\textbf{Eugene Syriani} is an Associate Professor at the Department of Computer Science and Operations Research at University of Montreal. He received his Ph.D. in Computer Science in 2011 from McGill University. His main research interests fall in software design based on the model-driven engineering approach, the engineering of domain-specific languages, model transformation and code generation, simulation-based design, collaborative modeling, and user experience. Contact him at http://www-ens.iro.umontreal.ca/~syriani.

==> commands.tex <==
\newcommand{\sem}[1]{\ensuremath{\llbracket #1 \rrbracket}}
\newcommand{\footnoteref}[1]{\textsuperscript{\ref{#1}}}
\newcommand{\defref}[1]{Definition~\ref{#1}}
\newcommand{\defrefName}[1]{\emph{\nameref{#1}}}
\newcommand{\figref}[1]{Fig.~\ref{#1}}
\newcommand{\Eqref}[1]{Equation~\ref{#1}}
\newcommand{\lstref}[1]{Listing~\ref{#1}}
\newcommand{\tabref}[1]{Table~\ref{#1}}
\newcommand{\chpref}[1]{Chapter~\ref{#1}}
\newcommand{\secref}[1]{Section~\ref{#1}}
\newcommand{\appref}[1]{Appendix~\ref{#1}}
\newcommand{\algoref}[1]{Algorithm~\ref{#1}}
\newcommand{\secrefFromTo}[2]{Sections~\begin{NoHyper}\ref{#1}--\ref{#2}\end{NoHyper}}

\newcommand{\secrefAndSecref}[2]{Sections~\ref{#1} and \ref{#2}}
\newcommand{\todo}[1]{
    \ifthenelse{\equal{#1}{}}{\textcolor{red}{TODO}}{\textcolor{red}{TODO:~{#1}}}
}

\newcommand{\algorithmicoutput}{\textbf{Returns:}}
\newcommand{\Returns}{\item[\algorithmicoutput]}


\newcommand\pname{AFP\xspace}
\definecolor{yellow}{RGB}{255,255,0}
\newcommand{\review}[1]{\noindent{\color{blue}{\textbf{Review: {#1}}}}}
\newcommand{\remark}[1]{\noindent{\colorbox[RGB]{255,230,230}{\parbox{\textwidth}{\textbf{Remark: {#1}}}}}}
\renewcommand{\nb}[2]{
	\fcolorbox{gray}{yellow}{\bfseries\sffamily\scriptsize#1}
	{\sf\small$\blacktriangleright$\textit{#2}$\blacktriangleleft$}
}


%%%%%%%%%% In-text commenting %%%%%%%%%%
\newcommand\id[1]{\noindent\nb{ID}{\textcolor{red}{#1}}}
\newcommand\es[1]{\noindent\nb{ES}{\textcolor{red}{#1}}}

\newcommand{\ugh}[1]{\textcolor{red}{\uwave{#1}}} % please rephrase
\newcommand{\ins}[1]{\textcolor{blue}{#1}} % please insert
\newcommand{\del}[1]{\textcolor{red}{\sout{#1}}} % please delete
\newcommand{\chg}[2]{\textcolor{red}{\sout{#1}}{\ra}\textcolor{blue}{\uline{#2}}} % please change

\newcommand{\newtextcolor}{purple2}
\newcommand\fix[1]{\textcolor{red}{#1}}
\newcommand\rem[1]{\textcolor{red}{\st{#1}}}
\newcommand\rep[2]{\textcolor{red}{\st{#1}}~\add{#2}}
\newcommand\add[1]{\textcolor{\newtextcolor}{{#1}}}


\newcommand\newtext[1]{\textcolor{\newtextcolor}{#1}}

\setul{0.5ex}{0.3ex}
\definecolor{purple}{RGB}{235, 52, 225}
\definecolor{purple2}{RGB}{232, 3, 252}
\setulcolor{purple}
\newcommand\phrasing[1]{\ul{#1}}

\newcommand{\todoref}{\textbf{{\color{orange}[ref?]}}}

%%%%%%%%%% Abbreviations %%%%%%%%%%

\newcommand{\ie}{i.e.,\xspace}
\newcommand{\eg}{e.g.,\xspace}
\newcommand{\etc}{etc.\xspace}
\newcommand{\etal}{\emph{et~al.}\xspace}

%%%%%%%%%% Names %%%%%%%%%%
\newcommand{\lowkey}{{\fontfamily{lmss}\selectfont lowkey}}

%%%%%%%%%% LWW types %%%%%%%%%%
\newcommand{\lwwregister}{\texttt{LWWRegister}}
\newcommand{\lwwset}{\texttt{LWWSet}}
\newcommand{\lwwmap}{\texttt{LWWMap}}
\newcommand{\lwwgraph}{\texttt{LWWGraph}}
\newcommand{\lwwvertex}{\texttt{LWWVertex}}
\newcommand{\lwwedge}{\texttt{LWWEdge}}

%%%%% TABLES %%%%%%%
\def\harveyBallsSize{0.75ex}

\newcommand*\rot{\rotatebox{0}}

==> listing.tex <==
\usepackage{listings}
\usepackage{color}

\definecolor{darkgreen}{rgb}{0,0.6,0}
\definecolor{gray}{rgb}{0.5,0.5,0.5}
\definecolor{mauve}{rgb}{0.58,0,0.82}
\definecolor{gray}{rgb}{0.4,0.4,0.4}
\definecolor{darkblue}{rgb}{0.0,0.0,0.6}
\definecolor{lightblue}{rgb}{0.0,0.0,0.9}
\definecolor{cyan}{rgb}{0.0,0.6,0.6}
\definecolor{darkred}{rgb}{0.6,0.0,0.0}
\definecolor{armygreen}{rgb}{0.29, 0.33, 0.13}
\definecolor{antiquefuchsia}{rgb}{0.57, 0.36, 0.51}
\definecolor{coolblack}{rgb}{0.0, 0.18, 0.39}


%basicstyle=\linespread{0.9}\scriptsize\ttfamily,

\lstset{
    basicstyle=\linespread{0.95}\footnotesize\ttfamily,
    columns=fullflexible,
    numberblanklines=false,
    numbers=left,                   % where to put the line-numbers
    numberstyle=\tiny\color{gray},  % the style that is used for the line-numbers
    stepnumber=1,
    numbersep=5pt,                  % how far the line-numbers are from the code
    backgroundcolor=\color{white},      % choose the background color. You must add \usepackage{color}
    showspaces=false,               % show spaces adding particular underscores
    showstringspaces=false,         % underline spaces within strings
    showtabs=false,                 % show tabs within strings adding particular underscores
    frame=none,                   % adds a frame around the code
    rulecolor=\color{black},        % if not set, the frame-color may be changed on line-breaks within not-black text (e.g. comments (green here))
    tabsize=2,                      % sets default tabsize to 2 spaces
    captionpos=b,                   % sets the caption-position to bottom
    breaklines=true,                % sets automatic line breaking
    breakatwhitespace=false,        % sets if automatic breaks should only happen at whitespace
    %  title=\lstname,                 % show the filename of files included with \lstinputlisting;
    xleftmargin=1.4em,              % align numbers with paragraph
    commentstyle=\color{darkgreen}\upshape,
    stringstyle=\color{darkred}
}

\lstdefinelanguage{XML}
{
    morestring=[s][\color{antiquefuchsia}]{"}{"},
    morestring=[s][\color{black}]{>}{<},
    morecomment=[s]{<?}{?>},
    morecomment=[s][\color{darkgreen}]{<!--}{-->},
    stringstyle=\color{black},
    identifierstyle=\color{darkred},
    keywordstyle=\color{darkred},
    morekeywords={xmlns,xsi,noNamespaceSchemaLocation,type,id,x,y,source,target,version,tool,transRef,roleRef,objective,eventually},% list your attributes here
    emph=[1]{name,implicit,grammarName,grammarType,library},
    emphstyle=[1]{\color{armygreen}}
}

\lstdefinelanguage{Xtext}
{
    morestring=[s][\color{darkred}]{'}{'},
    identifierstyle=\color{black},
    morekeywords={def,FOR,ENDFOR,IF,ENDIF},
    keywordstyle=\color{lightblue},
    emph=[1]{Function,RFID125,BranchRFID125,ReadCodeRFID125,WriteCodesRFID125,Concept,Attribute,SubType,Reference,Containment,Textual,Graphical,AttributeType},
    emphstyle=[1]{\color{armygreen}},
    emph=[2]{pin1,pin2,pin,codes,attributes,relation,super,ref_from,container,attrType,representation,conceptName},
    emphstyle=[2]{\color{antiquefuchsia}},
    emph=[3]{STRING,ID},
    emphstyle=[3]{\color{coolblack}},
    extendedchars=true
}

\lstdefinelanguage{Command}
{
    comment=[l]{--},
    morekeywords={READ,OBJECTS,CREATE,LINK,UPDATE,DELETE,TO},
    keywordstyle=\color{darkblue}\bfseries,
    morestring=[s][\color{darkred}]{\{}{\}},
    extendedchars=true
}

==> packages.tex <==
\usepackage[utf8]{inputenc}
\usepackage{pdftexcmds}
\usepackage[T1]{fontenc}
\usepackage{fancyvrb}
\usepackage{lipsum}
\usepackage{cite}
\usepackage{arydshln}
\usepackage[nomessages]{fp}% http://ctan.org/pkg/fp
\usepackage{url}
\usepackage{mdframed}
\usepackage{amsmath,amsfonts,amsthm} % Math packages
\usepackage{xcolor}
\usepackage{float}
\usepackage{subcaption}
\usepackage{enumitem}
\usepackage{nameref}
\usepackage{tabularx}
\usepackage{graphicx}
\usepackage{amsmath}
\usepackage{longtable}
\usepackage{array}
\usepackage{stmaryrd}
\usepackage{color}
\usepackage[outline]{contour}
\usepackage{colortbl,multirow,hhline}
\usepackage{tcolorbox}
\usepackage{booktabs}
% \hypersetup{
%     colorlinks = false,
%     linkbordercolor = {white}
% }
% \usepackage[hang, small,labelfont=bf,up,textfont=it,up]{caption} % Custom captions under/above floats in tables or figures
\usepackage{rotating}
\usepackage{harveyballs}
\usepackage{multirow}
\usepackage{afterpage}
\usepackage{epsfig}
\usepackage{xspace}
\usepackage{epsf,picinpar}
\usepackage{varioref}
\usepackage{listings}
\usepackage{amssymb}
\usepackage{pifont}
\usepackage{graphicx}
\usepackage[normalem]{ulem} % for \sout
\usepackage{multicol}
\usepackage[strings]{underscore}
\usepackage{balance}
\usepackage{framed}
\usepackage{textcomp}
\usepackage{parcolumns}
\usepackage{ifthen}
\usepackage{soul}
\usepackage{fancyvrb}

\usepackage{algpseudocode}
\usepackage{footmisc}
\usepackage{mathtools}
